Accurate ground state- and quasiparticle energies: beyond the RPA and GW methods with adiabatic exchange-correlation kernels

We review the theory and application of adiabatic exchange-correlation (xc-) kernels for ab initio calculations of ground state energies and quasiparticle excitations within the frameworks of the adiabatic connection fluctuation dissipation theorem and Hedin's equations, respectively. Various different xc-kernels, which are all rooted in the homogeneous electron gas, are introduced but hereafter we focus on the specific class of renormalized adiabatic kernels, in particular the rALDA and rAPBE. The kernels drastically improve the description of short-range correlations as compared to the random phase approximation (RPA), resulting in significantly better correlation energies. This effect greatly reduces the reliance on error cancellations, which is essential in RPA, and systematically improves covalent bond energies while preserving the good performance of the RPA for dispersive interactions. For quasiparticle energies, the xc-kernels account for vertex corrections that are missing in the GW self-energy. In this context, we show that the short-range correlations mainly correct the absolute band positions while the band gap is less affected in agreement with the known good performance of GW for the latter. The renormalized xc-kernels offer a rigorous extension of the RPA and GW methods with clear improvements in terms of accuracy at little extra computational cost.

==> cover.tex <==
Dear Editor

The submitted manuscript is a comprehensive review on the application of adiabatic non-local exchange-correlation kernels to obtain ground state- and quasi-particle energies in the framework of time-dependent density functional theory. The method constitutes is a natural generalization of the Random Phase approximation (RPA) and it is shown that the accuracy is dramatically increased compared to both RPA and standard GW calculations for ground state- and quasi-particle energies respectively. We provide several examples of applications including atomization energies of solids and molecules, van der Waals bonded systems, oxide formation energies, dissociation of dimers, surface- and chemisorption energies, structural parameters and quasi-particle energies of bulk and two-dimensional semiconductors. In all cases we report a significant increase in accuracy compared to state-of-the art calculations. Importantly, the methodology is universal, does not rely on fitted parameters, and yields accurate predictions for a diverse palette of electronic structure problems.

To our knowledge no other methodology in electronic structure theory can compete with the present approach in terms of accuracy and universality. For all the applications considered so far, the method produces results in close proximity to experimental values and in contrast to commonly applied electronic structure methods, the reliability does not depend on prior experience and benchmarks. The method is computationally demanding, but due to the ever increasing computational capabilities of supercomputers, we believe that the method will play a decisive role for electronic structure theory in the future. The manuscript is thus expected be of significant interest to anyone working in the field of electronic structure theory and should warrant publication in a high level specialized journal such as npj Computational Materials.

The manuscript also constitutes the May 2019 Psi_k highlight.

